Random Recurrent Neural Networks Dynamics

This paper is a review dealing with the study of large size random recurrent neural networks. The connection weights are selected according to a probability law and it is possible to predict the network dynamics at a macroscopic scale using an averaging principle. After a first introductory section, the section 1 reviews the various models from the points of view of the single neuron dynamics and of the global network dynamics. A summary of notations is presented, which is quite helpful for the sequel. In section 2, mean-field dynamics is developed. The probability distribution characterizing global dynamics is computed. In section 3, some applications of mean-field theory to the prediction of chaotic regime for Analog Formal Random Recurrent Neural Networks (AFRRNN) are displayed. The case of AFRRNN with an homogeneous population of neurons is studied in section 4. Then, a two-population model is studied in section 5. The occurrence of a cyclo-stationary chaos is displayed using the results of \cite{Dauce01}. In section 6, an insight of the application of mean-field theory to IF networks is given using the results of \cite{BrunelHakim99}.

==> MFAnalog.tex <==
%------------------------------------------------------------
\section{Mean-field dynamics for analog networks } \label{MFAnalog}
%------------------------------------------------------------

We are interested in the stationary dynamics of large
random recurrent neural networks. Moreover since we want to study
the meaning of oscillations and of (deterministic) chaos observed
in the finite sized models (see paper I), the regime of low noise
is specially interesting since the oscillations are practically
canceled if the noise is too strong. For these reasons, we cannot be
practically satisfied by  obtaining the limit $\mu_T$ of the
empirical measures. So we shall extract from $\mu_T$ dynamical
informations on the asymptotics of the network trajectories. Notice
that the distribution of the connexion weight distribution is not
necessarily Gaussian as long as it satisfies hypothesis
(H:\ref{H.hypo}).

\input{MFDHN}
\input{MFD2Pop}


==> MFD2Pop.tex <==
\subsection{Mean-field dynamics of 2-population AFRRNN} \label{MFD2Pop}
%---------------------------------------------------------
\subsubsection{2-population AFRRNN model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As it was announced previously, the assumption of a homogeneous
connexion weight model is not plausible. Besides, in literature,
RRNN models with several neuron populations have been studied as
early as in 1977 with \cite{Amari77} and have been thoroughly
investigated in the last decade (see for instance
\cite{Hansel96}). The heterogeneity of neuron population induces
interesting and complex dynamical phenomena such as
synchronization.
Actually the mean-field theory that was developed  in the
previous sections may be extended without major difficulty to
several neuron populations. To give a practical idea of what can be
obtained such extensions we consider here two populations with
respectively $N_1=\la N$ and $N_2=(1-\la)N$ neurons where
$\la\in]0,1[$ and where $N\ra\infty$.

Four connexion random matrices have to be considered in this model
$\J_{11}, \J_{12},\J_{21},\J_{22}$ where $\J_{ij}$ is the matrix
of connexion weights from population $j$  to population $i$.
 The random matrix $\J_{ij}$ is a $(N_j\times N_i$) random
matrix with independent identically distributed entries. Their
distribution is governed by statistical parameters
$(\oups_{ij},\ups_{ij})$ and obeys hypothesis (\ref{H.hypo}).
They are independent altogether.

However, the technical hypothesis (H) does not allow us to give to connexion
weights a rigorously constant sign, permitting to distinguish between inhibitory
and excitatory neurons. Indeed, there is no probability
distribution on \textit{positive} (resp. negative) real numbers, having a
 mean and a variance
respectively scaling as $\frac{\oups}{N}$ and
$\frac{\ups}{N}$. Thus, the positivity of the support induces on
the other side of the distribution a heavy tail which will not
respect assumption (iii) in hypothesis (H). However, it is possible
to consider probability distributions which are checking hypothesis
(H) and which are loading the negative numbers (or alternatively)
the positive ones) with arbitrary small probability.

We consider here a 2-population model with a population of
excitatory neurons and a population of inhibitory neurons (up to
the above restriction).

\subsubsection{General mean-field equations for moments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A large deviation principle may be obtained for the
2-population model for Gaussian connexion weights. So, the
convergence in finite time to the mean-field dynamics is shown,
in the present model with the same proof as in the previous 1-population model. See
\cite{Moynot99} for a rigorous proof and \cite{Dauce01} for a more
practical statement of results.
The limit of the empirical measure is the law of a Gaussian vector
which takes its values in $\F\times\F$. Each factor stands to
describe the repartition of a neural population. Note that the two
components are independent. As for the 1-population model we note
$m_k(t),q_k(t),c_k((s,t)$ the mean, variance and covariance at
given times of the empirical measure of population $k$
($k\in\{1,2\}$). The mean-field evolution equation for these
moments is described by the following system:

\begin{equation}\label{MFE2pop.eq}\left\{\begin{array}{lll}
m_k(t+1)=\sum_{j\in\{1,2\}}\oups_{kj}\int
f[\sqrt{q_j(t)+\sig^2}\xi+m_j(t)-\ta_j]d\ga(\xi)
\\
q_k(t+1)=\sum_{j\in\{1,2\}}J_{kj}^2\int
f[\sqrt{q_j(t)+\sig^2}\xi+m_j(t)-\ta_j]^2d\ga(\xi)
\\
c_k(s+1,t+1)=
{\Di\sum_{j\in\{1,2\}}}J_{kj}^2\int
f\left(\sqrt{\frac{[q_k(s)+\sig^2][q_k(t)+\sig^2]
-c_k(s,t)^2}{q_k(t)+\sig^2}}\xi_1
+\frac{c_k(s,t)}{\sqrt{q_k(t)+\sig^2}}\xi_2+m_k(s)-\ta_k\right)\times\\
\times f[\sqrt{q_k(t)+\sig^2}\xi_2+m_k(t)-\ta_k]d\ga(\xi_1)d\ga(\xi_2)
\end{array}\right.\end{equation}

\subsubsection{Results and discussion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  As far as numerical studies are concerned, we choose the following
values  for the statistical parameters
%
\begin{equation}
\left\{\begin{array}{cccc}
\oups_{1,1}=& gd &\hspace{2cm} J_{1,1}= &g
\\
  \oups_{1,2}= & -2gd &\hspace{2cm} J_{1,2}= & \sqrt{2}g
\\
  \oups_{2,1}= & gd &\hspace{2cm} J_{2,1}= &g
\\
  \oups_{22}= & 0 &\hspace{2cm} J_{22}= &0
\end{array}\right.
\end{equation}

In this study, according to some biological scheme,
excitatory neurons are connected both to excitatory neurons and
inhibitory neurons and inhibitory neurons are both connected to
excitatory neurons.   Moreover, the number of parameters is
reduced to allow numerical exploration of the synchronization
parameter. We keep two independent parameters:
\begin{itemize}
\item $g$ stands for the non linearity of the transfer function
\item $d$ stands for the differentiation of the two populations
(inhibitory vs. excitatory).
\end{itemize}

Considering the firing thresholds as previously, there is no
variation about individual thresholds. Excitatory neuron threshold
$\ta_1$ is chosen equal to 0 and inhibitory neuron
threshold $\ta_2$ is chosen equal to 0.3 because the
activation potential of inhibitory neurons is always positive.

In the bifurcation map of \ref{fig:bifurmap} (extracted from
\cite{Dauce01}) several dynamical regimes are displayed and the
corresponding numerical ranges of parameters $d$ and $g$ are
displayed. Notice that theoretical previsions of the mean-field
equations (\ref{MFE2pop.eq}) and the large scale simulations of
large-sized  networks behavior are consistent.

 As in the homogeneous
case there is a transition to chaos for weak $d$. When the differentiation
parameter $d$ is sufficiently large (about 2), the fixed point looses its
stability through a Hopf bifurcation to give rise to synchronous
oscillations when $g$ is growing. There is then a succession of bifurcations
leading to chaos (see paper I).

Moreover, a new phenomenon occurs. For large $g$, there is a significant transition
regime between stationary chaos and synchronized oscillations
which is named "\textit{cyclo-stationary chaos}". In that regime,
statistical parameters are exhibiting regular periodic
oscillations, though individual trajectories are diverging
with a mean quadratic distance behaviour which is characteristic
from chaos.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Ins=E9rer figure de IJCNN 2000
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[height=8cm,width=12cm,clip=false]{Figures/bifurmap}
\caption{Bifurcation map of the 2-population model}
\label{fig:bifurmap}
\end{center}
\end{figure}


